Falcon: Fair Active Learning using Multi-armed Bandits

Biased data can lead to unfair machine learning models, highlighting the importance of embedding fairness at the beginning of data analysis, particularly during dataset curation and labeling. In response, we propose Falcon, a scalable fair active learning framework. Falcon adopts a data-centric approach that improves machine learning model fairness via strategic sample selection. Given a user-specified group fairness measure, Falcon identifies samples from "target groups" (e.g., (attribute=female, label=positive)) that are the most informative for improving fairness. However, a challenge arises since these target groups are defined using ground truth labels that are not available during sample selection. To handle this, we propose a novel trial-and-error method, where we postpone using a sample if the predicted label is different from the expected one and falls outside the target group. We also observe the trade-off that selecting more informative samples results in higher likelihood of postponing due to undesired label prediction, and the optimal balance varies per dataset. We capture the trade-off between informativeness and postpone rate as policies and propose to automatically select the best policy using adversarial multi-armed bandit methods, given their computational efficiency and theoretical guarantees. Experiments show that Falcon significantly outperforms existing fair active learning approaches in terms of fairness and accuracy and is more efficient. In particular, only Falcon supports a proper trade-off between accuracy and fairness where its maximum fairness score is 1.8-4.5x higher than the second-best results.

==> entropy.tex <==

\section{Trial-and–error Labeling Strategy}
\label{sec:trialanderror}
The problem has now changed to selecting examples from the target groups when the labels are not available. A straightforward approach for coping with unknown labels is to generate pseudo labels and choose samples with the highest informativeness. Indeed, there is a heavy literature on their generation. If the pseudo labels are perfect, then we would not have to postpone using samples at all. However, there is a fundamental limit in the correctness as we show in our experiments.

Our solution is to select samples that are likely to be informative and label them, but postpone using them for training when they turn out to have undesirable labels. Later on if we actually need these labels to further improve fairness or accuracy, we can use them. This approach may sound counter-intuitive because labeling is expensive, and we are not using them. However, using them at this point can actually negatively affect fairness, so it is better not to use them. Here we show how trial-and-error labeling can guarantee fairness improvement for demographic parity (DP) and equal opportunity (EO), and refer readers to Appendix X for other measures.
\begin{example} Demographic Parity (DP). Continuing from Example X, 
\end{example}

\begin{example} \Equal opportunity (EO). Continuing from Example X, 
\end{example}

\section{Selecting Informative Samples}
\label{sec:informativesamples}
We now discuss how to select samples that are the most informative, but also have a label of interest. Informativeness can be measured in several ways, and we use an information theoretic approach using Shannon’s entropy. The information obtained by a sample labeled as $x$, $I(x)$ can be expressed as follows:
\[
I(x) = p \log \frac{1}{p} + (1 - p) \log \frac{1}{1-p}
\]
where $p$ is the predicted probability of being label 1 by the trained model. The first term means the expected information score when $x$ is labeled 1, and the second term means the expected information score when the label is 0. If we draw a plot, we get a concave curve that peaks when $x = 0.5$. Intuitively, if $x$ is closer to 0 or 1, we have a lower risk of mislabeling and thus obtain smaller information as well. 

Unlike traditional active learning, we only get the partial information score with our trial-and-error labeling strategy, so selecting $p=0.5$ examples is no long the best solution. For example, if the target group is label 1, we will postpone label 0 data and do not obtain any information on label 0, so the information I(x) now becomes $p \log \frac{1}{p}$ ($I(x) =(1 - p) \log \frac{1}{1-p}$ for target label 0). Hence, a point near $p=1/e \approx 0.367$ instead of $p=0.5$ would be most useful for improving the accuracy of target label 1 ($1-1/e \approx 0.632$ for target label 0).

However, $p$ value is not the same as the actual accuracy because the model prediction is not always accurate, especially for the AL setting where there is a little amount of training data. Even if we pick the points with $p=0.3$, it does not mean that 30\% of examples always have a ground truth label 1. Therefore, directly optimizing the partial information score is not an optimal solution either.



==> problem_old.tex <==
\section{Problem Definition and Overview}

The goal is to choose samples that when labeled maximize both model fairness and accuracy. For illustrative purposes, we now assume two sensitive groups (i.e., $\mathbb{Z} = \{0, 1\}$), and discuss extensions to multiple sensitive groups later. 
% \kt{think about multiple classes. how to define target groups \& control aggressiveness in this case.}

% For now, we assume binary classes and two sensitive groups and discuss extensions to multiple classes and sensitive groups later.

We give an overview of the \method{} framework. As an input, the user provides a group fairness measure. Then \method{} determines which ``target'' groups of samples need to be labeled first. This approach is more general than class imbalance works with fixed minority groups where the minority groups themselves may change as samples are labeled and do not need to have fewer examples. When selecting samples for a specific group, the selection itself may be incorrect due to the lack of labels, so \method{} learns the right policy to select samples that are informative and yet are not likely to end up having incorrect labels. We discuss the technical details of \method{}'s workflow in the following sections. 

\begin{figure}[h]
\centering
  \includegraphics[width=\columnwidth]{figures/overview.pdf}
  \caption{Overview of \method{} workflow.}
  \label{fig:overview}
\end{figure}
